Motion Planning for Autonomous Driving: The State of the Art and Future Perspectives

Intelligent vehicles (IVs) have gained worldwide attention due to their increased convenience, safety advantages, and potential commercial value. Despite predictions of commercial deployment by 2025, implementation remains limited to small-scale validation, with precise tracking controllers and motion planners being essential prerequisites for IVs. This paper reviews state-of-the-art motion planning methods for IVs, including pipeline planning and end-to-end planning methods. The study examines the selection, expansion, and optimization operations in a pipeline method, while it investigates training approaches and validation scenarios for driving tasks in end-to-end methods. Experimental platforms are reviewed to assist readers in choosing suitable training and validation strategies. A side-by-side comparison of the methods is provided to highlight their strengths and limitations, aiding system-level design choices. Current challenges and future perspectives are also discussed in this survey.

==> SubSection/ModelFormulation.tex <==
\section{Problem Formulation}
\subsection{Pipeline Planning Methods}
The pipeline method also named the modular approach, is widely used by the industry and is nowadays considered the conventional approach. This method is mainly divided into Global Route Planning and Local Behavior/Trajectory Planning. 
\subsubsection{Global Route Planning}
\subsubsection{Local Behavior/Trajectory Planning}

\subsection{End-to-End Planning Methods}
\subsubsection{Imitation Learning}
\subsubsection{Reinforcement Learning}
\subsubsection{Parallel Planning}

==> Tables/ImitationTable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{ccccll}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Article}               & \textbf{Category} & \textbf{Raw Data}                                             & \textbf{Dataset\Platform}                                   & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Implement Tasks}}     & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Detail}}                                                                                                                                              \\ \hline
Codevilla et al. \cite{IL5}    & \textbf{BC}       & Monocular image                                               & Carla Branchmark                                            & Simulation navigation task                                               & Use high-level commands as a switch to select the appropriate branch                                                                                                                                     \\
Chen et al. \cite{IL_Inter1}   & \textbf{BC}       & Monocular image                                               & TORCS Dataset and KITTI                                     & Simulation navigation task                                               & Embedded an affordance into model, the affordance learns from perception data and is used to predict control actions                                                                                     \\
Sauer et al. \cite{IL_Inter2}  & \textbf{BC}       & Monocular video and directional input                         & Carla Branchmark                                            & Physical navigation task, handle traffic light and speed signs           & Conditional affordance is trained to calculate low-dimension intermediate representations from video and high-level command                                                                              \\
Zeng et al. \cite{IL_Inter4}   & \textbf{BC}       & Lidar data and HD Map                                         & Physical Dataset collected in North America                 & \textbf{Physical Navigation Task with trajectory-3D Detection as output} & Propose the first learnable and interpretable end-to-end motion planner, leverage intermediate representations to improve the interpretability of the end-to-end model                                   \\
Sadat et al. \cite{IL_Inter5}  & \textbf{MMM}      & Lidar data and HD Map                                         & Physical Dataset collected in North America                 & Physical navigation task                                                 & Propose a joint system for self-driving vehicles including perception, prediction, and motion planning, which can produce interpretable intermediate representations.                                    \\
Ross et al. \cite{IL8}         & \textbf{DPL}      & Monocular image                                               & A 3D racing game and Super Mario Bros                       & Autonomous racing competition and character control                      & Propose an iterative algorithm, which learns a stationary deterministic policy guaranteed to perform well under its induced distribution of states                                                       \\
Zhang et al. \cite{IL10}       & \textbf{DPL}      & Monocular image                                               & A racing car simulator, named TORCS and its dataset         & Autonomous racing competition                                            & Embedded query-efficient model to further reduce the requirement for the label in expert trajectories.                                                                                                   \\
Yan et al. \cite{IL12}         & \textbf{DPL}      & LiDAR, ego-vehicle speed, and Relative Sub-goal               & Physical and Simulate robot platform                        & Physical and simulation navigation task                                  & Fuse the novice policy and the expert policy to control the robot with a quantified safe criterion.                                                                                                      \\
Li et al. \cite{OIL}           & \textbf{DPL}      & Monocular image and sub-goal                                  & Sim4CV Platform                                             & Autonomous racing competition                                            & Provide a reward-based online learning method for multiple experts which allows learning optimal control policies from sub-optimal expert trajectories.                                                  \\
Ohn-Bar et al. \cite{LSD}      & \textbf{DPL}      & Monocular image                                               & Carla Branchmark                                            & Simulation navigation task                                               & Embedded scenario context network into policy learning network, and both networks are optimized by online iterative training strategy                                                                    \\
Levine et al. \cite{BIRL2}     & \textbf{BM}       & BEV image for simulation environment                          & Highway driving simulator, three Way, constant speed        & Keep the lane, change lanes and takeover                                 & Leverage the Gaussian algorithm to learn the reward function and determine the relevance of features which is presented in the expert trajectory.                                                        \\
Brown et al. \cite{BIRL3}      & \textbf{BM}       & Monocular image                                               & Driving simulator                                           & Keep the lane, change lanes and takeover                                 & Propose a sampling method based on Bayesian inverse reinforcement learning and calculate the practical high-confidence upper bounds on the α-worst-case difference by expert   trajectories.             \\
Palan et al. \cite{BIRL4}      & \textbf{BM}       & Monocular image                                               & Lunar lander simulator                                      & Keep the lane, change lanes and takeover                                 & Propose a probabilistic method based on maximum entropy, and provides a well-defined, globally normalized reward function for decision sequences problem                                                 \\
Ziebart et al. \cite{MEIRL}    & \textbf{MEM}      & Road network, Sub-goal, and GPS Data                          & Driver route modeling                                       & Long range autonomous navigation task                                    & Develop a probabilistic approach based on the principle of maximum entropy and provide a well-defined, globally normalized distribution over decision sequences.                                         \\
Lee et al. \cite{MEIRL4}       & \textbf{MEM}      & Monocular image                                               & the Next Generation Simulation (NGSIM) and Carla Branchmark & Keep the lane, change lanes and takeover                                 & Leverage the expert trajectory to learn a coarse reward function and use the demonstrations to ground the query generation process.                                                                      \\
Ho et al. \cite{MEIRL5}        & \textbf{MEM}      & Monocular image                                               & Carla Branchmark                                            & Keep the lane, change lanes and takeover                                 & Integrate Generative Adversarial Network (GAN) to IRL, treat the expert trajectory as a true label, and then approximate the expert policy by generating adversarial training                            \\
Phan-Minh et al. \cite{Extend} & \textbf{MEM}      & Mid-level representation, HD map, other obstacles information & Autonomous driving dataset from the Las Vegas Strip         & Autonomous driving in real-life state with heavy traffic                 & Propose an IRL planner with three steps, generate a set of proposed trajectories, filter trajectories with an interpretable safety filter, then leverage a network to score each   remaining trajectory. \\ \hline

\end{tabular}
\end{table}
